First-order tree-to-tree functions

We study tree-to-tree transformations that can be defined in first-order logic or monadic second-order logic. We prove a decomposition theorem, which shows that every transformation can be obtained from prime transformations, such as tree-to-tree homomorphisms or pre-order traversal, by using combinators such as function composition.

==> atomic-and-combinators.tex <==



==> figure-fot.tex <==

\newcommand{\simplefunfig}[4]{
    \begin{tabular}{cc}
        $\ranked{
        \xymatrix@C=1.5cm{
#2 \ar[r]^-{#1}& #3
        }}$
        \\
        {#4}
    \end{tabular}   
 }

 \newcommand{\reversiblefunfig}[4]{
    \begin{tabular}{cc}
        $\ranked{
        \xymatrix@C=1.5cm{
#2 \ar@<.5ex>[r]^-{#1}& #3
\ar@<.5ex>[l]
        }}$
        \\
        {#4}
    \end{tabular}   
 }



 \newcommand{\laterfunfig}[3]{
    \begin{tabular}{cc}
        $\ranked{
        \xymatrix@C=1.5cm{
#1 & #2
        }}$
        \\
#3
    \end{tabular}   
 }
 



\begin{figure}
    \begin{tabular}{cc}
        \simplefunfig
        {\iota_i}
        {\Sigma_i}
        {\Sigma_1 + \Sigma_2}
        {$a \mapsto (a,i)$}
        &
        \simplefunfig
        {\mathrm{forget}}
        {\Sigma+\Sigma}
        {\Sigma}
        {$(a,i) \mapsto a$}
        \\ \\ 
        % \\ \\
        % \reversiblefunfig
        % {\mathrm{swap}}
        % {\Sigma \product \Gamma}
        % {\Gamma \product \Sigma}
        % {$\tensorpair{a,b} \mapsto \tensorpair{b,a}$}
        % &
        \simplefunfig
        {\distrtensor}
        {\reduce k (\Sigma_1 + \Sigma_2)}
        {\reduce k \Sigma_1 + \reduce k \Sigma_2}
        {$(a,i)/f \mapsto ((a/f),i)$}
         & 
        \reversiblefunfig
        {\distrtensor}
        {(\Sigma_1 + \Sigma_2)\product \Gamma}
        {(\Sigma_1 \product \Gamma) + (\Sigma_2 \product \Gamma)}
        {$\tensorpair{(a,i),b} \mapsto (\tensorpair{a,b},i)$}
        \\ \\
        \reversiblefunfig
        {\distrtensor}
        {\shallowterm {(\Sigma_1 + \Sigma_2)} \Gamma}
        {(\shallowterm {\Sigma_1} \Gamma) + (\shallowterm {\Sigma_2} \Gamma)}
        {$(a,i)\tensorpair{b_1,\ldots,b_n} \mapsto (a\tensorpair{b_1,\ldots,b_n})$ }
        &
        \reversiblefunfig
        {\distrtensor}
        {\shallowterm {(\Sigma_1 \product \Sigma_2)} \Gamma}
        {(\shallowterm {\Sigma_1} \Gamma) \product (\shallowterm {\Sigma_2} \Gamma)}
        {
        \begin{tabular}{c}
            $\tensorpair{a_1,a_2}\tensorpair{b_1,\ldots,b_n} \mapsto$ \\
            $\tensorpair{a_1 \tensorpair{b_1,\ldots,b_{n_1}}, a_2\tensorpair{b_{n_1+1},\ldots,b_n} }$  \\
            where $n_1$ is the arity of $a_1$
        \end{tabular}    
        }
        \\ \\
        \reversiblefunfig
        {}
        {\rSigma}
        {\shallowterm 1 {\tmonad \Sigma}}
        {$a \mapsto 1.\tensorpair a$}
        &
        \reversiblefunfig
        {\composeterm}
        {1 + \shallowterm \Sigma {\tmonad \Sigma} }
        { \tmonad \Sigma}
        {
        \begin{tabular}{c}
            Every term is either just a port,\\ or has a root and child subterms.    
        \end{tabular}    
        } 
        \\ \\
        \simplefunfig
        {}
        {\Sigma}
        {\reduce k \Sigma}
        {$a \mapsto a/(i \mapsto (1,i))$ } &
        \simplefunfig
        {}
        {\reduce {k_1} \reduce {k_2} \Sigma}
        {\reduce {k_1 \cdot k_2} \Sigma}
        {$(a/f)/g \mapsto a/(g \circ f)$}
        \\ \\
        \simplefunfig
        {\unit_\Sigma}
        {\Sigma}
        {\tmonad \Sigma}
        {\tablepic{69}}
        & 
        \\ \\
        \simplefunfig
        {\flatt_\Sigma}
        {\tmonad \tmonad \Sigma}
        {\tmonad \Sigma} 
        {\tablepic{73}}
        &
        \simplefunfig
        {\distrtf}
        { \tmonad \reduce 1 \Sigma}
        {\reduce 1 \tmonad \Sigma}
        {\tablepic{74}}
        \\ \\
        \laterfunfig
        {\tmonad(\Sigma_1+\Sigma_2) \ar@<.5ex>[r]^{ \ancfact}
        \ar@<-.5ex>[r]_{\decfact}}
        {\tmonad(\tmonad \Sigma_1 + \tmonad \Sigma_2)} 
        {see Section~\ref{sec:prime-and-combinators}} 
        &
        \laterfunfig
        {\tmonad \Sigma \ar[r]^-{\preorder}}
        {\reduce 1 \tmonad(\rSigma + 0 + 2)}
        {see Section~\ref{sec:prime-and-combinators}} 
        \\ \\ 
        \laterfunfig
        {\shallowterm{(\reduce k \Sigma)}{\Gamma^k} \ar[r]^-{\unfold}}
        {(\shallowterm \Sigma \Gamma)^k}
        {see Section~\ref{sec:prime-and-combinators}} 
    \end{tabular} 
    \caption{    \label{fig:fo-term}The prime functions. The functions are parametrised by types  $\rSigma, \ranked{\Sigma_1}, \ranked{\Sigma_2}, \rGamma$. In the above, the type $\ranked i$ for $i \in \set{0,1,2}$ represents a  ranked set   with one element of arity $i$. Some of the functions are bijections, as indicated by double arrows, in these cases both the function and its inverse are prime functions. }
\end{figure}




==> matrix-power.tex <==

\section{Matrix power} 
\label{sec:matrix-power}
In this section, we define the matrix power, which can be seen as a way of representing several trees in one. %Roughly speaking, the several trees are the contents of registers in a register automaton.
%, and the single tree that represents them is the computation tree of the register automaton.  We then show that several trees stored in a computation  can be unfolded in a derivable way. 

\begin{definition}
    [Matrix power] For $k \in \set{1,2,\ldots}$ define the $k$-th matrix power\footnote{
        The name  matrix power is based the matrix power in  universal algebra (for the latter, see~\cite{Taylor1975} or~\cite{szendrei1990simple}). Roughly speaking, the restrictions that we place on the original definition correspond to the single-use and monotone conditions from Definition~\ref{def:stt}. 
     } of a ranked set $\rSigma$ 
to be 
\begin{align*}
 \mati k \rSigma \quad \eqdef \quad \ranked{\reduce k \rSigma^k}.
\end{align*}
\end{definition}

Here is a picture of a binary element in the matrix power, where $k=3$:
\begin{center}
\includegraphics[scale=.4, page=85]{pics.pdf}
\end{center}

A matrix power of arity $n$ is used as an abstraction of an $n$-ary register update $\ranked{R\to \tmonad(\Gamma+R+\dots+R)}$. The number $k$ represents the number of registers (that is the size of $\ranked {R}$), and each letter from $\rSigma$ represents a register update (that is, an element of $\ranked{\tmonad(\Gamma+R+\dots+R)}$). When two letters share the same port in the matrix power, this means that the corresponding register updates call the same component of $\ranked{R+\dots+R}$ in their definition, the position in the fold indicates which precise register is called. For instance, the register update above is an abstraction of the following binary register update of registers $r, s$ and $t$:
   \begin{center}
   \includegraphics[scale=.3]{register-update-matrix-power.pdf}
   \end{center}
When we run a STT on an input tree, we decorate it with register updates following the transition function. In order to evaluate this tree, the first thing to do is to determine, for each register update of the root, its "dependency tree" that is to say the register updates they call, inductively. When register updates are abstracted by matrix powers, this operation of determining the dependency tree is what we call \emph{unfolding}. We illustrate it by the following example 
\begin{center}
\includegraphics[scale=.38]{unfold-matrix-power}
\end{center}
Formally, \emph{unfolding} is a function of type
\begin{align*}
    \ranked{\unfold : \tmonad \mati k \rSigma \to \mati k {(\tmonad \Sigma)} }
    \end{align*}
 which is defined as follows by induction on the size of the input term. If the input is an empty term, then the output is this term:
\begin{center}
\includegraphics[scale=.3, page=83]{pics.pdf}
\end{center}
Otherwise, if the input is a nonempty term $a(t_1,\ldots,t_n)$ then the output is obtained by first applying unfolding to to the smaller terms $t_1,\ldots,t_n$, and then applying the following derivable function, which we call \emph{shallow unfold}. 
\begin{align*}
    \ranked{
        \xymatrix{
            \shallowterm{\mati k \rSigma} {\mati k \rGamma}  \ar[r] & \mati k {(\shallowterm \Sigma \Gamma)}.
        }
    }
\end{align*}
Here is a picture of unfolding for shallow terms:
\begin{center}
\includegraphics[scale=.4]{unfold-shallow}
\end{center}
More formally, unfolding for shallow terms is defined to be   the composition of the following functions
    \begin{align*}
        \xymatrix@R-1pc@C=3.2cm{
          {\begin{array}{c}
          \shallowterm{\mati k \rSigma} {\mati k \rGamma} \\{=\shallowterm{\reduce k {\Sigma^k}}{\reduce k {\Gamma^k}}}
          \end{array}}  \ar[d]_{{\mathrm{Commutativity}}}\ar[r]^{\mathrm{Shallow\  unfold}} &  {\begin{array}{c}
         \ranked{\mati k {(\shallowterm \Sigma \Gamma)}} \\=  \ranked{ \reduce k(\shallowterm{\Sigma}{ {\Gamma}})^k}
          \end{array}} \\
             \reduce k(\shallowterm{\reduce k {\Sigma^k}}{ {\Gamma^k}})  \ar[r]_{{\mathrm{Matching}}} &  \ranked{ \reduce k(\shallowterm{\Sigma^k}{ {\Gamma}}) } \ar[u]_{\mathrm{Commutativity}} 
        } 
    \end{align*}
Since our prime functions and combinators do not have any general mechanisms for induction, it is not clear how to derive the unfolding operation. In fact, it is not derivable in general, but it will become derivable after imposing a monotonicity requirement. The need for this condition is shown in Example~\ref{eq:twist}.  Let us define it in the following.

For a port $i$ in an element of the matrix power $a/f \in \mati k \rSigma$ define its \emph{twist} to be the partial function from $\set{1,\ldots,k}$ to itself 
which is the composition of 
\begin{align*}
\xymatrix{
    [1,k] \ar[r]^-{j \mapsto {(j,i)}} & [1,k] \times [1,n] \ar[r]^-{f^{-1}} & [1,\arity a] \ar[r] & [1,k]
}
\end{align*}
where the last function maps each port of the tuple $a$ to the coordinate of the tuple that created that port. Here is a picture:
\begin{center}
\includegraphics[scale=.3, page=87]{pics.pdf}
\end{center}
 We say that an element of the $k$-matrix power is \emph{monotone} if all of its ports have monotone twist. For instance, the right example above is not monotone.
 We are now ready to state the principal result of this section.

\begin{proposition}\label{prop:monotone-unfold}
    For every finite ranked set $\rSigma$ and every $k \in \set{1,2,\ldots}$ there is a derivable function 
    \begin{align*}
    \ranked{ f : \tmonad \mati k \Sigma \to \mati k {(\tmonad \Sigma)}}
    \end{align*}
    which coincides with term unfolding for monotone inputs.
\end{proposition}
The proof of the  above lemma is one of the main technical contributions of this paper, and it is given in the appendix. One of the ingredients of the proof is a first-order (in fact, derivable) version of the Factorisation Forest Theorem for trees, which is based in Colcombet's splits from~\cite{colcombetCombinatorialTheoremTrees2007}.  

%\begin{corollary}\label{cor:matrix-power}
%    Let $\rSigma$ be a finite set and let $\rDelta \subseteq \mati k \rSigma$ be a finite set which contains only monotone elements. Then one can derive the tree-to-tree function
%    \begin{align*}
%    f : \trees \rDelta \to \trees \rSigma  \qquad t \mapsto \text{first tree in the unfolding of $t$.}
%    \end{align*}
%\end{corollary}
% Let $\alg$ be an algebra and let $k \in \set{1,2,\ldots}$. How should the $k$-th power of the algebra be defined? For the domain, we use  $k$-tuples from the domain of $\alg$.  What about the operations? A natural   approach is to define the $n$-ary operations to be  $k$-tuples of $n$-ary operations from $\alg$, acting coordinate-wise. Because of the coordinate-wise action,  the coordinates in the product are independent of each other. This will be insufficient for our intended application, where the algebra $\alg$ is meant to represent individual register automaton, since the contents of register $r$ in the output of a register update depend on the contents of other registers in the input valuation . To  model this interdependence, we use a more sophisticated notion of power, 
% defined below.
% \begin{definition}
%     For an algebra $\alg$ and $k \in \set{1,2,\ldots}$, the $k$-th matrix power\footnote{
%         The definition of matrix power that we use is a special case of the original definition of matrix power from universal algebra (for the latter, see~\cite{Taylor1975} or~\cite{szendrei1990simple}). Roughly speaking, the restrictions that we place on the original definition correspond to the single-use and monotone conditions from Definition~\ref{def:stt}. 
%     } of $\alg$ is defined as follows. The domain and signature are defined by
%     \begin{align*}
%     \overbrace{(\algdom \alg)^k}^{\text{domain}} \qquad \overbrace{
%         \ranked{\reduce k ((\algops \alg)^k)}}^{\text{signature}}
%         \end{align*}
%         while the  shallow product operation is defined by
%         \begin{align*}
%             \ranked{
%         \xymatrix{
%             \shallowterm {\reduce k (\algops \alg)^{k}} {{(\algdom \alg)}^k} \ar[d] \\
%             \shallowterm {(\algops \alg)^{k}} {{(\algdom \alg)}} \ar[d] \\
%             (\shallowterm {(\algops \alg)} {{(\algdom \alg)}})^k
%          \ar[d]\\
%             (\algdom \alg)^k
%         }
%         }
%         \end{align*}
% \end{definition}

% By definition, if an algebra has a derivable shallow product, then the same is true for its  matrix powers, i.e.~for every $k$ the shallow product in the $k$-th matrix power is derivable. The following proposition -- which is much harder to show -- states a similar implication for  (not necessarily shallow) products.  
% \begin{proposition}\label{prop:matrix-power} If an algebra has a derivable product, then the same is true for its matrix powers.
% \end{proposition}
%




==> need-for-monotonicity.tex <==
\subsection{The need for monotonicity in the unfolding}
\begin{example}\label{eq:twist}
    Consider the following elements in a second matrix power:
\begin{center}
\includegraphics[scale=.3, page=84]{pics.pdf}
\end{center}
Let $t_n \in \trees \mati 2 \rSigma$ be the tree which consists of a path with $n$ nodes using the unary label $a$, followed by a leaf with label $b$. If we apply term unfolding to this tree, and then project to the first coordinate, then we get a tree with a white leaf if and only if  $n$ is even.  If term unfolding were derivable, then thanks to the results from Section~\ref{sec:to-transductions}  we would get a first-order tree-to-tree transduction 
\begin{align*}
\trees \redset{a,b} \to \trees \rSigma
\end{align*}
where the output would contain a white leaf if and only if the input has odd depth. This is in turn would imply that having even depth for trees over $\redset{a,b}$ is first-order definable, which it is not, because first-order logic cannot do modulo counting.
\end{example}
The problem in the above example is that the letter $a$ does a swap on its ports, which leads to counting modulo two. To forbid such swaps, we impose a monotonicity requirement that matches the monotonicity requirement for register updates in register transducers.


==> prelims.tex <==

\section{First-order tree functions}
The goal of this paper is to describe the first-order tree-to-tree functions as the smallest class which contains certain prime functions, and which is closed under applying certain combinators. To achieve this goal, we discuss functions that transform not just trees, but also \emph{terms}, which are trees with distinguished ports that can be substituted with trees (or other terms). One of the main points of using terms is that  they have a substitution structure, i.e.~one can build a terms of terms. 

\paragraph*{Types.} In the end we are interseted about tree-to-tree functions. However, to construct such functions, we will use intermediate operations which transform terms,  pairs of terms, or terms of terms, etc.
 The following definition describes the types that can be used by the intermediate operations.



\begin{definition}[Types]\label{def:types}
    Define a \emph{type} to be any ranked set which can be obtained from the prime types by applying the type constructors, as described below. We denote by $\Tt$ the set of all types. 
    \begin{itemize}
        \item {\bf prime types.} 
           \begin{enumerate}
            \item every ranked set with finitely many elements;
            \item a ranked set, call it  $\llone$, which has one element on every arity;
        \end{enumerate}
    \item {\bf Type constructors.} 
     \begin{enumerate}
        \item {\bf Disjoint union $\Sigma+\Gamma$.} An element of $\Sigma+\Gamma$ is either an element of $\Sigma$ or an element of $\Gamma$, with the arities inherited from $\Sigma,\Gamma$. 
        \item {\bf Cartesian\footnote{This is the Cartesian product in the category where objects are ranked sets, and morphisms are arity preserving functions.}  product $\Sigma \times \Gamma$.} An  $n$-ary element of $\Sigma \times \Gamma$ is a pair of elements from $\Sigma, \Gamma$, respectively, whose arities are both $n$.
        \item {\bf Terms.} For a ranked set  $\Sigma$, define a \emph{term}\footnote{The terms that we use are special kinds of terms, where each variable is used exactly once.} to be tree over the alphabet $\Sigma + \set \portletter$, where $\portletter$ is a fresh symbol of arity zero. Define $\terms \Sigma$ to be the ranked set of terms over $\Sigma$, where the arity of a term is the number of labels $\portletter$.
\item {\bf Matrix power $\Sigma^{[k]}$.} An $n$-ary element of $\Sigma^{[k]}$ is a list of $\Sigma$ elements $[\sigma_1,\dots,\sigma_k]$ of lenght $k$, together with a function $f$ of the following type:
\[f: \cup_{i\leq k} \sigma_i\times [1, \mathsf{ar}(\sigma_i)]\to [1,n]\times [1,k]\]
which describes how to connect each output of each symbol $\sigma_i$ to an output of the global $\Sigma^{[k]}$ symbol (this is the first component of the image of $f$) and in which order (this is the second component), as illustrated by Fig.~\ref{FigMatrixPower}.

\begin{figure}

\caption{Example of an element of $\Sigma^{[k]}$\label{FigMatrixPower}}
\end{figure}

Moreover, $f$ should satisfy the following two conditions\footnote{These conditions are necessary to capture the fo fragment. We will relax them later to capture other logic such as chain logic or mso.}:
\begin{itemize}
\item {\bf Single use contraint.} $f$ is a bijection;
\item  {\bf Bottom-up monotonicity.} If $i<i'$ and $f(\sigma_i, o)=(m,l)$ and $f(\sigma_{i'},o')=(m,l')$ then $l<l'$. 
\end{itemize}

%\item {\bf Tensor product $\Sigma \product \Gamma$.} An  $n$-ary element of $\Sigma \product \Gamma$ is a pair of elements from $\Sigma, \Gamma$, respectively, whose arities  sum up to $n$. \textcolor{red}{No need for tensor. }
%
    \end{enumerate}  
    \end{itemize}  
\end{definition}

\newcommand{\tensorpair}[2]{\langle #1, #2 \rangle}

%The tensor constructor can be seen as a special case of the term constructor, since a tensor pair $\tensorpair a b$  can be viewed as a tree of depth two like in this picture:
%\begin{center}
%    (picture)
%\end{center}
%In fact, the term constructor can be viewed as a least fixpoint of tensor products, as expressed in the following isomorphism:
%\begin{align*}
%    \terms \Sigma \quad \simeq \quad  \set \portletter + \coprod_{a \in \Sigma} \underbrace{\terms \Sigma \product \cdots \product \terms \Sigma}_{\text{arity of $a$ times}}
%\end{align*}


\paragraph*{prime functions.} Having described the types, we now describe the prime functions that transform elements of these types.




\begin{definition}[prime functions]\label{def:prime-functions} The \emph{prime functions} are the following functions (for every types $\Sigma,\Gamma,\Sigma_0,\Sigma_1$): 
\begin{enumerate}
    \item The unique arity-preserving function $! : \Sigma \to \llone$
    \item Every arity-preserving function $f : \Sigma \to \Gamma$ such that    $\{x \in \Sigma \ \mid \ f(x)\neq x\}$ is finite. In particular, every finite domain arity-preserving function $f : \Sigma \to \Gamma$ and the identity function $f : \Sigma \to \Sigma$.
    \item Projection and co-projection:
    \begin{align*}
        \pi_i : \Sigma_0 \times \Sigma_1 \to \Sigma_i \qquad \iota_i : \Sigma_i \to \Sigma_0 + \Sigma_1
    \end{align*}
    \item Distribution of $+$ across $\times$:
\begin{align*}
    (\Sigma_0 + \Sigma_1 ) \times \Gamma \to (\Sigma_0 \times \Gamma) + (\Sigma_1 \times \Gamma)
\end{align*}
\item Distribution of $+$ across $\product$:
\begin{align*}
    (\Sigma_0 + \Sigma_1 ) \product \Gamma \to (\Sigma_0 \product \Gamma) + (\Sigma_1 \product \Gamma)
\end{align*}
\item Flattening:
\begin{align*}
    \sf{Flat}: \terms \terms \Sigma \to \terms \Sigma
\end{align*}
\item Blocking
    \begin{align*}
        \sf{Block}^{\uparrow}:\terms (\Sigma + \Gamma) \to \terms (\terms \Sigma + \terms \Gamma)\\
        \sf{Block}^{\downarrow}:\terms (\Sigma + \Gamma) \to \terms (\terms \Sigma + \terms \Gamma)
    \end{align*}
    \item Depth first search
    \begin{align*}
        \sf{DFS}:\terms \Sigma \to \terms (\Sigma+\llone)
    \end{align*}
    \item Unfolding: 
\begin{align*}
    \sf{Unfold}:\terms \Sigma^{[k]} \to (\terms \Sigma)^{[k]}
\end{align*}
Be aware that we should prove that the image of an element from $\terms \Sigma^{[k]}$ is indeed an element of $(\terms \Sigma)^{[k]}$, in particular that the function $f$ is bijective and bottom-up monotonic. The second property can be proved by induction on the lenght of the path connecting the root to the output..
    \item Unit:
\begin{align*}
    \sf{Unit}:\Sigma  \to \terms \Sigma
\end{align*}

%\item Assuming that $\Sigma$ is finite, the two canonical bijections (one in each direction) between the ranked sets:
% \begin{align*}
%    \terms \Sigma \qquad \text{and} \qquad    \set \portletter + \coprod_{a \in \Sigma} \underbrace{\terms \Sigma \product \cdots \product \terms \Sigma}_{\text{arity of $a$ times}}
%\end{align*}

\end{enumerate}
\end{definition}



The prime functions can be combined into more complex functions using the following combinators.
\begin{definition}
     [Combinators] \label{def:combinators} \ 
    \begin{enumerate}
    \item Function composition:
    \begin{align*}
    \frac{f : \Sigma \to \Gamma \quad g : \Gamma \to \Delta} {g \circ f : \Sigma \to \Delta}
\end{align*}

\item Lifting functions to trees:
\begin{align*}
    \frac{f : \Sigma \to \Gamma} {\terms f : \terms \Sigma \to \terms \Gamma}
\end{align*}
\item Cases
\begin{align*}
    \frac{f_0 : \Sigma_0 \to \Gamma \quad f_1 : \Sigma_1 \to \Gamma} {[f_0,f_1] : \Sigma_0 + \Sigma_1 \to \Gamma}
\end{align*}

\item Pairing functions:
\begin{align*}
    \frac{f_0 : \Sigma \to \Gamma_0 \quad f_1 : \Sigma \to \Gamma_1} {(f_0,f_1) : \Sigma \to \Gamma_0 \times \Gamma_1}
\end{align*}

%\item Tensor product of functions:
%\begin{align*}
%    \frac{f_0 : \Sigma_0 \to \Gamma_0 \quad f_1 : \Sigma_1 \to \Gamma_1} {\langle f_0,f_1 \rangle : \Sigma_0 \product \Sigma_1 \to \Gamma_0 \product \Gamma_1}
%\end{align*}
\end{enumerate}
\end{definition}

We are now ready to define the first-order tree functions, which are the topic of this paper. 

\begin{definition}[First-order tree functions] \label{def:fo-tree-functions} \ 
    \begin{itemize}
        \item A \emph{first-order term functions} is any function that can be  generated from the prime functions from Definition~\ref{def:prime-functions} by applying the  combinators from Definition~\ref{def:combinators}.
        \item  A \emph{first-order tree function} is any first-order term function restricted to trees, i.e.~terms of arity zero.
    \end{itemize}    
\end{definition}
%\begin{remark}
Note that first-order term functions are arity preserving. 
%\end{remark}

To illustrate these first-order tree functions, we present a series of examples, many of which will be useful later.

\bigskip
%\noindent \begin{example}[Identity] For every type $\Sigma$, the identity function $x\in\Sigma\mapsto x\in\Sigma$ is a first-order tree function. This is achieved by induction on the types: the identity function over a finite set of elements is first-order since its domain is finite, and the identity function over $\llone$ is the first-order function $!$. For $\Sigma$ and $\Gamma$ in $\Tt$ , the identity
%function over $\Sigma+\Gamma$ is the disjoint union of the co-projections $\Sigma \to \Sigma + \Gamma$ and $\Gamma \to \Sigma + \Gamma$. The
%identity function over $\Sigma \times \Gamma$ is the pairing of the projections $\Sigma \times \Gamma \to \Sigma$ and $\Sigma \times \Gamma \to \Gamma$. The
%identity function over $\Sigma \product \Gamma$ is the tensor product of the identity over $\Sigma$ and the identity over $\Gamma$. Finally,
%the identity function over $\terms\Sigma$ is constructed from the identity function over $\Sigma$ using the combinator $\terms$.
%\end{example}
%
%
%\bigskip
\noindent\begin{example}[Filter] Let $\Gamma, \Sigma\in\Tt$, where $\Gamma$ is a finite set of unary symbols. Consider the function:
$$ f:\terms (\Sigma+\Gamma)\to\terms \Sigma$$
which erases the elements of $\Gamma$ from the inupt tree. This function is well defined since erasing unary symbols does not break the tree structure of the input. 
Let us explain why this is a first-order list function. 
Consider the function $unit:\Sigma\to\terms\Sigma$ and the constant function $Empty:\Gamma\to\terms\Sigma$ which associates to every element of $\Gamma$ the empty tree. The function $Empty$ is a first order tree function since its domain is finite. Using the cases combinator, we get a tree in $\terms\terms\Sigma$, which we transform into a tree in $\terms \Sigma$ using flattening.
\end{example}

\bigskip
\noindent \begin{example}[If then else] Let $\llzero$ be another copy of the type $\llone$. Suppose that $f : \Sigma \to \llzero+\llone$ and $g_0, g_1 : \Sigma \to\Gamma$ are first-order tree functions. Then the function:
 \begin{align*}
  g\colon \Sigma &\to \Gamma \\
  x &\mapsto g_0(x)  \text{ if } f(x)\in\llzero\\
  x &\mapsto g_1(x)  \text{ if } f(x)\in\llone.
\end{align*}
 is also a first-order tree function. This is done as follows. On input
$x\in\Sigma$, we first apply the pairing of f and the identity function, yielding a result:
$$ (f(x),x)\in(\llzero+\llone)\times\Sigma$$
Next we apply the function distribute, transforming the type into:
$$ \llzero\times\Sigma+\llone\times\Sigma$$
To this result we apply the disjoint union $h_0 + h_1$ where $h_0:\llzero\times\Sigma\to \Gamma$ and
$h_1:\llone\times\Sigma\to \Gamma$ are defined by $h_i=\pi_2(id_i,g_i)$, where $id_0$ and $id_1$ are the identity function on $\llzero$ and $\llone$ respectively, yielding the desired result.
\end{example}



\bigskip
\noindent \begin{example}[Siblings and parent information]
Let $\Gamma$ be a finite type, and $n$ the maximal arity of its symbols. We set $\Gamma^{\sf{Sib}}$ to be the ranked set where an $n$-ary symbol is either an $n$-ary symbol of $\Gamma$ or a pair of an $n$-ary symbol of $\Gamma$ together with a list of lenght at most $n$ of elements from $\Gamma+\bot$. % Adding $\Gamma$ is useful in the proof, step 7

\medskip
Consider the function:
\[ Sib: \terms \Gamma \to \terms (\Gamma^{\mathsf{Sib}})\]
which tags every node of a tree in $\terms \Sigma$ by the list of its siblings (the missing siblings are witnessed by $\bot$ in the list).

% from  $(\Gamma\cup\bot)^{\leq n}$, whose lenght is the arity of the node, and such that the $i^{th}$ element of the  list is the symbol of its $i^{th}$ sibling if it has one, otherwise it is $\bot$.
Let us explain why $Sib$ is a first-order tree function. 
\begin{enumerate}
\item For every symbol $a\in \Gamma$, consider the unary symbols $a_\#$ and $a_\flat$.
We set $\Gamma_\#=\{a_\#\mid a\in\Gamma\}$ and $\Gamma_\flat=\{a_\flat\mid a\in\Gamma\}$.
Let $g$ be the following function:
 \begin{align*}
  g\colon \Gamma &\to \terms(\Gamma+\Gamma_\#+\Gamma_\flat)\\
  a &\mapsto a_\#[a[a_\flat,\dots,a_\flat]].
\end{align*}
The action of $g$ on a $\Gamma$ symbol looks like this:
\begin{center}
Picture
\end{center}
\item We lift $g$ to the trees of $\terms \Gamma$ using the combinator $\terms$, then apply a flattenig. After this operation, a tree in $\terms\Gamma$ is transformed to a tree in $\terms(\Gamma+\Gamma_\#+\Gamma_\flat)$ this way:
\begin{center}
Picture
\end{center}
\item We apply $\sf{Block}^{\uparrow}$, to separate the symbols of $\Gamma$ form the symbols of $\Gamma_\#+\Gamma_\flat$, we get then a tree in $\terms(\terms\Gamma+\terms(\Gamma_\#+\Gamma_\flat))$. Those trees look like this:
\begin{center}
Picture
\end{center}
\item Consider the function $h:\terms(\Gamma_\#+\Gamma_\flat)\to \terms(\Gamma_\#+\Gamma_\flat)$ which transforms the trees of the following shape as follows:
\begin{center}
Picture
\end{center}
and leaves the others unchanged. 
The function $h$ is a first-order tree function because it is not the identity only in a finite set.

\item To the blocks $\terms \Gamma$ we apply the identity function, and to the blocks $\terms(\Gamma_\#+\Gamma_\flat)$ we apply $h$. After that, we apply a flettening to get trees in $\terms(\Gamma+\Gamma_\#+\Gamma_\flat)$ of the form:
\begin{center}
Picture
\end{center} 
\item We apply block to separate the symbols of $\Gamma_\flat$ form the others. Doing so, every $\Gamma$ node ends up in the same block as its siblings (marked with $\#$):
\begin{center}
Picture
\end{center}
\item Consider the function $k:\terms(\Gamma+\Gamma_\#)\to \terms(\Gamma^{\sf{Sib}}+\Gamma_\#+\Gamma_\flat)$ which transforms every tree of the following shape as follows:
\begin{center}
Picture
\end{center}
and leaves the other unchanged. We apply the function $k$ to the $\terms(\Gamma+\Gamma_\#)$
blocks and the injection $\terms (\iota_1\circ \iota_1):\terms(\Gamma_\flat)\to \terms(\Gamma^{\sf{Sib}}+\Gamma_\#+\Gamma_\flat)$ to the other $\terms(\Gamma_\flat)$ blocks. Then we apply a flattening and erase the symbols from $\Gamma_\#+\Gamma_\flat$. Doing so we get the desired function.
\end{enumerate}
\medskip

Let $\Gamma$ be a finite type. We set $\Gamma^{\sf{Par}}$ to be the ranked set where an $n$-ary symbol is either an $n$-ary symbol of $\Gamma$ or a pair of an $n$-ary symbol of $\Gamma$ together with a list of lenght at most $1$ of elements from $\Gamma$. % Adding $\Gamma$ is useful in the proof, step 7

\medskip
Now consider the function $$Par:\terms\Gamma\to \terms (\Gamma^{\sf{Par}})$$ which adds to every node of a tree in $\terms \Sigma$ the list (of lenght at most 1) containing the symbol of its parent. In particular, its root is labeled by the empty list. 
The fuction $Par$ is a first order tree function. To see this, the same steps above can be followed, exept for steps 6 and 7 which should be adapted this way:
\begin{enumerate}
\item[6'] We apply block to separate the symbols of $\Gamma_\#$ form the others. Doing so, every $\Gamma$ node ends up in the same block as its parent (marked with $\flat$):
\begin{center}
Picture
\end{center}
\item[7'] Consider the function $k:\terms(\Gamma+\Gamma_\flat)\to \terms(\Gamma^{\sf{Sib}}+\Gamma_\#+\Gamma_\flat)$ which transforms every tree of the following shape as follows:
\begin{center}
Picture
\end{center}
and leaves the other unchanged. We apply the function $k$ to the $\terms(\Gamma+\Gamma_\flat)$
blocks and the injection $\terms (\iota_0\circ \iota_1):\terms(\Gamma_\#)\to \terms(\Gamma^{\sf{Sib}}+\Gamma_\#+\Gamma_\flat)$ to the other $\terms(\Gamma_\#)$ blocks. Then we apply a flattening and erase the symbols from $\Gamma_\#+\Gamma_\flat$. Doing so we get the desired function.
\end{enumerate} 
\end{example}



\bigskip
\noindent  \begin{example}[Root and leaves] Let $\Sigma$ be a finite type and $f:\Sigma \to \Gamma$, $g: \Sigma \to \Gamma$ be first order tree functions. 

The function $\sf{root}_{f,g} : \terms\Sigma \to \terms\Gamma$
which applies $f$ to the root and $g$ to the rest of the tree is a first order tree function.
 
To show this, we first start by applying the function $Par:\terms\Sigma\to\terms(\Sigma^{\sf{Par}})$ to the trees of $\terms \Sigma$. Doing so, the root can be distinghished from the other nodes since it will be tagged by the empty list, while the other nodes will be tagged by lists of lenght exactly $1$. We denote by $\Sigma^\emptyset$ the set of $\Sigma^{\sf{Par}}$ symbols tagged by the empty list. 

Consider the functions $f_{\sf{root}}: \Sigma^\emptyset\to \Gamma$, the restriction of $f$ to $\Sigma^\emptyset$; and $g_{\neg\sf{root}}: \Sigma^{\sf{Par}}\setminus\Sigma^\emptyset\to \Gamma$, the restriction of $g$ to $\Sigma\setminus\Sigma^\emptyset$. Both are fo tree functions since they are arity preserving and have finite domain.
By applyin the cases combinator to $f_{\sf{root}}$ and $g_{\neg\sf{root}}$ and lifting the obtained function to trees, we obtain $\terms{[f_{\sf{root}}, g_{\neg\sf{root}}]}: \terms{\Sigma^{\sf{Par}}}\to \terms \Gamma$, which, composed with $Par$, gives the desired function $\sf{root}_{f,g}$.

\medskip
The function $\sf{leaves}_{f,g} : \terms\Sigma \to \terms\Gamma$
 which applies $f$ to the leaves and $g$ to the rest of the tree is a first order tree function. This is done using the same ideas as before, but invoquing the function $Sib$ instead of the function $Par$: leaves can be distingushed from the other nodes since they are tagged by lists of $\bot$. \end{example}

\bigskip
\noindent\begin{example}[Descendent and ancestors]
If $\Sigma$ is a finite type, we set $\Sigma_{\sf{Bool}}$ to be the ranked set whose elements are the elements of $\Sigma$ tagged by $0$ or $1$. 
\begin{itemize}
\item The function $\sf{Desc}_\Gamma: \terms \Sigma \to \terms (\Sigma_{\sf{Bool}})$ which 
adds $1$ to the label of each node depending on whether it has a descendent in $\Gamma\subseteq \Sigma$.
\item The function $\sf{Anc}_\Gamma: \terms \Sigma \to \terms (\Sigma_{\sf{Bool}})$ which 
adds $1$ to the label of each node depending on whether it has an ancestor in $\Gamma\subseteq \Sigma$.
\end{itemize}

We set in the rest of this example $\Delta$ to be $\Sigma\setminus\Gamma$.
To show that $\sf{Desc}_\Gamma$ and $\sf{Anc}_\Gamma$ are first order tree functions, let us notice first that the following four functions are fo tree functions:
\[h_{X,i}:\terms X \to \terms \Sigma_{\sf{Bool}}\qquad X\in \{\Gamma,\Delta\}, i\in\{0,1\}\]
which taggs the nodes of $\terms X$ by $i$. 
Indeed, each function $h_{X,i}$ can be obtained by liftting the function $\sf{Tagg}_i:X\to\Sigma_{Bool}$, which taggs the elements of $X$ by $i$, to trees using the combinator $\terms$. The function $\sf{Tagg}_i$ is itself first order since it is arity preserving and finite domain.

To obtain the $\sf{Desc}_\Gamma$ function, we start by applying the $\sf{block}^{\downarrow}:\terms{(\Gamma+\Delta)}\to \terms{(\terms\Gamma+\terms\Delta)}$ function. Note that the blocks which should be assigned $0$ are exactly the $\terms \Delta$ blocks which are leaves. Let us consider the function $f:=[h_{\Gamma,1},h_{\Delta,0}]:\terms\Gamma+\terms \Delta\to \terms\Sigma_{\sf{Bool}}$ and $g:=[h_{\Gamma,1},h_{\Delta,1}]:\terms\Gamma+\terms \Delta\to \terms\Sigma_{\sf{Bool}}$. The function $\sf{Desc}_\Gamma$
is obtained by applying $f$ to the leaves and $g$ to the other nodes, then fy flattening the result.

\medskip
The function $\sf{Anc}_\Gamma$ is obtained in a similar way.    
\end{example}


We are now ready to state the main result of this paper. 
\begin{theorem}\label{thm:main}
    The following classes of functions are equal\begin{itemize}
        \item First-order tree-to-tree transductions;
        \item First-order tree functions.
    \end{itemize}
\end{theorem}

The bottom-up inclusion, i.e.~the proof that every first-order tree function is a first-order tree-to-tree transduction, is proved by induction in Section~\ref{sec:to-transductions}.  The bottom-up inclusion is true by design, i.e.~the prime functions and combinators were designed so that they could be easily  simulated using first-order transductions. 

The hard part of the theorem is showing that every first-order tree-to-tree transduction can be broken up, using the combinators, into the prime functions. The proof strategy for the hard part is presented in Section~\ref{sec:strategy}, and is then realised in Sections~\ref{sec:fo-translation} and~\ref{sec:one-register}.

==> strategy.tex <==
\section{Proof strategy}
\label{sec:strategy}
In this section, we present an overview of the top-down implication in the  proof of Theorem~\ref{thm:main}, which says that every first-order tree-to-tree transduction is (the restriction to trees of) a derivable function. The proof has five steps, which are spread across Sections~\ref{sec:fo-translation}--\ref{sec:stt-derivable}, and summarised below.

\newcommand{\announce}[2]{
\begin{center}
    {\bf #1.} #2
\end{center}
}
%\begin{enumerate}
%\item



  %  \item
  \paragraph*{Section~\ref{sec:fo-translation}: first-order tree relabellings.} We begin the proof of the left-to-right  implication  with a special case of first-order tree-to-tree transductions, which we call \emph{first-order  tree relabellings.} In such a  function, every node of the input tree  is given a new label, depending on first-order definable properties of the node. An example is:  ``if a leaf $x$ in the input tree has at least one ancestor with label $a$, then replace the label of $x$ with the letter $c$''. First-order tree relabellings  do not cover all first-order transductions, because they do not change the shape of the input tree, but they are an important subcase.
    The main result of Section~\ref{sec:fo-translation} is:
    \announce
    {Proposition~\ref{prop:forat}}
    {Every first-order tree relabelling is derivable.}
    The main tool used in the proof of Proposition~\ref{prop:forat} is a theorem of Schlingloff~\cite[Theorem 2.6]{schlingloff1992expressive}, which can be seen as tree version of Kamp's theorem about {\sc ltl} being  expressively complete for first-order logic.  
    
    

 \paragraph*{Section~\ref{sec:stt}: register transducers.} To prove that  first-order tree-to-tree transductions are derivable, it will be more convenient to use an automaton model. In Section~\ref{sec:stt}, we present  this  automaton model, which we call \emph{register transducers}\footnote{These are the only kind of register transducer used in this paper. A more complete name would be first-order tree-to-tree register transducers.}. This  is a bottom-up tree automaton, which uses registers to store parts of the output tree. The model is based on streaming tree transducers from~\cite{alur2017streaming}, but it is  appropriately restricted so that it matches first-order logic, as opposed to monadic second-order logic which was used in~\cite{alur2017streaming}. The main result of Section~\ref{sec:stt} is:
    \announce
    {Theorem~\ref{thm:stt}}
    {Every first-order  tree-to-tree transduction can be computed by a  register transducer.}
    The proof of the above theorem, like for similar results in~\cite{alur2017streaming} or~\cite[Theorem 23]{engelfrietMSODefinableString2001}, is based on the composition method in logic. 
    The converse implication is also true, and follows from Proposition~\ref{prop:many-register} and the bottom-up implication in Theorem~\ref{thm:main}.
    
     \paragraph*{Section~\ref{sec:one-register}: register transducers with one register.} By Theorem~\ref{thm:stt}, in order to prove the left-to-right implication in Theorem~\ref{thm:main}, it is enough to show that register transducers can only compute  derivable  functions. As a first step, we consider register transducers with only one register. When there is only one register, the computed function turns out to be a composition of a first-order tree relabelling, as treated  Proposition~\ref{prop:forat}, followed by the evaluation (i.e.~computation of the $\beta$-normal form) of    a simply typed $\lambda$-term which is affine (i.e.~uses each variable at most once). The main result of Section~\ref{sec:one-register} is that evaluation of  affine $\lambda$-terms is  derivable, as stated in the following theorem:
    \announce
    {Theorem~\ref{thm:normalise}}
    {The following function is derivable
    \begin{align*}
    \text{affine $\lambda$-term} \qquad \mapsto \qquad \text{its $\beta$-normal form,}
    \end{align*}
    if we restrict inputs so that they use  a fixed number of variables, and all subterms have types from a fixed finite set of simple types. }
    

\paragraph*{Section~\ref{sec:stt-derivable}: deriving a register transducer.}  In Section~\ref{sec:stt-derivable}, we complete the proof of Theorem~\ref{thm:main}:
    \announce
    {Proposition~\ref{prop:many-register}}
    {Every function computed by a register transducer is derivable.}
    The above result, together with Theorem~\ref{thm:stt}, completes the proof of the left-to-right implication in Theorem~\ref{thm:main}. The proof of Proposition~\ref{prop:many-register} is the observation that register automata with many registers can be reduced to register automata with one register, using the unfolding operation. For register transducers with one register only, the only computation that is done is iterated substitution, which is derivable thanks to Theorem~\ref{thm:normalise}.


==> stt-derivable.tex <==

\section{Functions computed by register transducers are derivable}
\label{sec:stt-derivable}
We now  have all of the ingredients needed to derive functions computed by register transducers, as stated in the following proposition.
\begin{proposition}
    \label{prop:many-register} 
For every first-order  tree transducer, the computed function is derivable. 
\end{proposition}
The above proposition  completes the proof of the left-to-right implication in Theorem~\ref{thm:main}: we have seen, by Proposition~\ref{prop:many-register}, that first-order tree-to-tree transductions can be computed by first-order tree transducers, and Proposition~\ref{prop:many-register} shows that the later are derivable, which concludes the proof.

The rest of this section is devoted to proving Proposition~\ref{prop:many-register}. There will be four main ingredients, namely derivability for: first-order tree relabelings (Proposition~\ref{prop:forat}), normalisation of affine $\lambda$-terms (Theorem~\ref{thm:normalise}), and unfolding of the matrix power (Proposition~\ref{prop:monotone-unfold}).
\label{sec:proof-of-prop} 
To put these ingredients together,  we use  terminology inspired by universal algebra, as given in the following definition. 

\begin{definition}
    An \emph{algebra} $\alg$ consists of two sets 
    \begin{align*}
    \overbrace{\algdom \alg}^{\text{unranked}} \qquad \overbrace{\algops \alg}^{\text{ranked}},
    \end{align*}
equipped with a  \emph{shallow product}\footnote{
    A more standard approach would be to use a family of operations indexed by the signature
    \begin{align*}
    \set{f^\alg : (\algdom \alg)^{\arity f} \to \algdom \alg}_{f \in \algops \alg}.
    \end{align*}
   Our approach is equivalent, i.e.~defining a shallow product is the same as defining a family of operations.
}, which is function of type
\begin{align*}
 \shallowterm {(\algops \alg)}{\underbrace{(\algdom \alg)}_{\substack{\text{viewed as a ranked}\\ \text{set, with all elements}\\ \text{having arity zero}}}} \rto \redpar {\algdom \alg}.
\end{align*}
    For an algebra $\alg$, define its \emph{product} to be the function of type
    \begin{align*}
        \treepar {\algops \alg} \to \algdom \alg
    \end{align*}
    defined in the natural way.
    %  An algebra is called \emph{derivable} if its product  is derivable. 
\end{definition}


One example of an algebra is when the signature is some ranked set $\rSigma$, the domain is  $\trees \rSigma$, and the interpretation is defined in the natural way. In this case, the product operation is the identity. A variant of this algebra is when the signature is replaced by $\tmonad \rSigma$; in this case the product operation becomes flattening. 

Let us begin the proof of Proposition~\ref{prop:many-register}.
Fix a register transducer with $k$ registers. For the rest of this section, when talking about register valuations and register updates, we mean the registers of the fixed register transducer.
Another example of an algebra was implicit in the definition of register transducers: the domain is the register valuations and the signature is the  register updates. To prove  Proposition~\ref{prop:many-register}, we will show that the algebra of register updates embeds -- via the matrix power -- in an algebra, call it $\alg$, whose product operation is derivable as a special case of normalisation of affine $\lambda$-terms. 
 The idea behind the algebra  $\alg$ is to use  $\lambda$-terms to represent register contents, according to the following picture:
 \begin{center}
 \includegraphics[scale=.3, page=59]{pics.pdf}
 \end{center}
%    \mypic{59}  
    Let  $\nmax$  be the maximal arity of registers in the fixed register transducer, and let  $\rGamma$ be its  output alphabet. For a term $t \in \tmonad \rGamma$ of arity at most $\nmax$, its representation as a  $\lambda$-term, which we denote by $t^\lambda$,  uses variables from the following finite set (we use the notation $\otype^i \to \otype$ defined in Example~\ref{ex:affine-not-enough}):
\begin{align*}
X  \quad \eqdef \quad \set{\typevar {x_a} {\otype^i \to \otype} : a \in \rGamma \text{ of arity $i$}} \cup \set{\typevar {x_i} \otype : i \in \set{1,2,\ldots,\nmax }}.
\end{align*}
Furthermore, $t^\lambda$ is affine and it can be typed using simple types  from  the following set finite set :
\begin{align*}
    \Tt \quad \eqdef \quad \set{\otype^i \to \otype : i \in \set{0,\ldots,\nmax}}
\end{align*}
This means that if $t$ has arity at most $\nmax$ -- which is true for any term that can appear in a register of our fixed register transducer -- then its $\lambda$-term representation $t^\lambda$ satisfies constraints as in Theorem~\ref{thm:normalise}.  On its own, $t^\lambda$ is already in normal form, so there is no need to normalise it, but we intend to compose  such $\lambda$-terms, leading to terms that are not in normal form (but which still use variables from $X$ and types from $\Tt$). 
This motivates the  following definition of an algebra, call it $\alg$. Its domain and signature are given by 
\begin{align*}
\overbrace{\set \bot + \trees \lamrank X}^{\algdom \alg}  \qquad \overbrace{ \tmonad \lamrank X}^{\algops \alg} 
\end{align*}
\begin{align*}
\text{where }\lamrank X = {\overbrace{\set{x : x \in X}}^{\text{arity 0}} \cup \overbrace{\set{\lambda x : x \in X}}^{\text{arity 1}} \cup  \overbrace{\set @}^{\text{arity 2}}}
\end{align*}
In other words, the domain is $\lambda$-terms plus an error element, and the signature is $\lambda$-terms  with ports. The   product operation is 
\begin{align*}
t^\alg(t_1,\ldots,t_n) = \begin{cases}
    \text{normal form of $t(t_1,\ldots,t_n)$} & \text{if $t(t_1,\ldots,t_n)$ is affine and can be typed using $\Tt$}\\
    \bot & \text{otherwise}
\end{cases}
\end{align*}
In particular, if one of the inputs $t_1,\ldots,t_n$ is $\bot$, then the output is also $\bot$.  The algebra $\alg$ is designed so that we can apply Theorem~\ref{thm:normalise} about normalising $\lambda$-terms to see that the  product operation in the  algebra $\alg$ is derivable. Next, by observing that the matrix power is a form of syntactic sugar for manipulating registers in a register automaton, we see that there is an arity preserving 
    \begin{align*}
    \ranked h : \regups \to \mati k {(\algops \alg)}
    \end{align*}
    which has only monotone elements in its image, and which makes the following diagram commute
    \begin{align*}
    \xymatrix@C=2cm{
        \treepar {\regups} \ar[r]^-{\trees \ranked h}\ar[d]_{\text{product}} &
         \treepar {\mati k {(\algops \alg)}}\ar[r]^{\text{Corollary~\ref{cor:matrix-power}}}  & 
         \treepar {\algops \alg} \ar[d]^{\text{product}} \\
        \regvalss \ar[rr]_{(t_1,\ldots,t_k) \mapsto t^\lambda_1}&  & \algdom {\alg^{[k]}}
    }
    \end{align*} 
Putting this all together, we see that there is a derivable function which inputs a tree of register updates, and outputs the value of the first register, represented as a $\lambda$-term. The last remaining observation is that function $t^\lambda \mapsto t$, i.e.~the inverse of the $\lambda$-term representation, is derivable. This inverse can be achieved, for example, by composing a first-order tree relabelling with a tree homomorphism. This completes the proof of Proposition~\ref{prop:many-register}, and therefore also of Theorem~\ref{thm:main}. 

==> to-transductions.tex <==
\newcommand{\Root}[1]{\mathsf{root}_{#1}}
\newcommand{\Port}[1]{\mathsf{port}_{#1}}
\newcommand{\Interface}[1]{\mathsf{Interface}_{#1}}
\section{Derivable functions are first-order transductions}
\label{sec:to-transductions}
In this section, we give an overview on the proof of the right-to-left implication in Theorem~\ref{thm:main}, namely that if $\rSigma,\rGamma$ are finite ranked sets, then for every derivable function $\ranked {f : \tmonad \rSigma \to \tmonad \rGamma}$, its restriction to trees $f : \trees \rSigma \to \trees \rGamma$
is a first-order tree-to-tree transduction. The proof is a simple induction on the derivation of  $\ranked f$. In the induction, we must deal with functions that manipulate types that are more complex than trees, e.g.~tensor pairs of terms of coproducts.  To operate on such types with first-order transductions, we need to show how such types can be modeled as relational structures. For this purpose, we associate to each type $\rSigma$
\begin{itemize}
\item a relational vocabulary denoted  \emph{voc$ \rSigma$};
\item a map $\underline{\bullet}: a \in \rSigma  \mapsto \underline a \in \text{models over voc$ \rSigma$}$;

    which interprets every inhabitant of $\rSigma$ as a relational structure over the vocabulary of $\rSigma$,
\end{itemize}
both defined in a natural way by induction on types. Their precise definition are given in  Definition~\ref{def:type-model}.
    \smallskip

The following proposition immediately yields the right-to-left implication in Theorem~\ref{thm:main}. Its proof, which is a straightforward case analysis of all prime functions and combinators, is in the appendix. 


  
\begin{proposition}\label{prop:to-logic} If $f : \rSigma \to \rGamma$ is derivable, then there is a first-order transduction $g$ 
    which makes the following diagram commute
    \begin{align*}
        \xymatrix@C=3cm{
            \rSigma \ar[d]_{a \mapsto \underline a}\ar[r]^f &  \rGamma \ar[d]^{a \mapsto \underline a} \\
            \text{models over  Voc$\rSigma$} \ar[r]_g &  \text{models over Voc$ \rGamma$}.
        } 
    \end{align*}
\end{proposition}





==> together.tex <==
\section{Putting it all together}
% Define a \emph{fo-translation} to be any function
% \begin{align*}
%     \trees \Sigma \to \trees \Gamma
% \end{align*}
% which is obtained by composing the characteristic functions of several unary fo-queries, and then applying a letter-to-letter renaming. 


Theorem~\ref{thm:main} follows immediately from the following lemma, and the results in the previous sections.

\begin{lemma}
    Every first-order tree-to-tree transduction is a finite composition of functions of the form:
    \begin{itemize}
        \item a relabelling, i.e.~a function $\tmonad f : \tmonad \sigma \to \tmonad \tau$ for some $f : \sigma \to \tau$ where $\sigma,\tau$ are finite ranked sets;
        \item a characteristic function as in Lemma~\ref{lem:fo-char};
        \item unfolding as in Lemma~\ref{lem:unfold};
        \item substitution as in Lemma~\ref{lem:substitute}
    \end{itemize}
\end{lemma}
\begin{pr}
    By understanding the semantics of a first-order definable streaming tree transducer.
\end{pr}  
